Testing neutrino spectra formation in collapsing stars with the diffuse supernova neutrino flux

I address the question of what can be learned from the observation of the diffuse supernova neutrino flux in the precision phase, at next generation detectors of Megaton scale. An analytical study of the spectrum of the diffuse flux shows that, above realistic detection thresholds of 10 MeV or higher, the spectrum essentially reflects the exponential-times-polynomial structure of the original neutrino spectrum at the emission point. There is only a weak (tens of per cent) dependence on the power \beta describing the growth of the supernova rate with the redshift. Different original neutrino spectra correspond to large differences in the observed spectrum of events at a water Cerenkov detector: for typical supernova rates, the ratio of the numbers of events in the first and second energy bins (of 5 MeV width) varies in the interval 1.5 - 4.3 for pure water (energy threshold 18 MeV) and in the range 1 - 2.5 for water with Gadolinium (10 MeV threshold). In the first case discrimination would be difficult due to the large errors associated with background. With Gadolinium, instead, the reduction of the total error down to 10-20 % level would allow spectral sensitivity, with a dramatic improvement of precision with respect to the SN1987A data. Even in this latter case, for typical neutrino luminosity the dependence on \beta is below sensitivity, so that it can be safely neglected in data analysis.

==> reply_to_referee.tex <==
Dear Editors, 

please receive the corrected version my paper DA10480/Lunardini, "Testing neutrino spectra formation in collapsing stars with the diffuse supernova neutrino flux".  I have made changes according to the referee's comments. 

Below I summarize the  changes made, and reply to the referee's remarks.

I hope that my paper is now ready for publication.  

Thank you, with best regards,

Cecilia Lunardini

------------------------------------------------------------

Summary of changes:

1. The sixth paragraph of the introduction has been slightly modified
   in reply to a comment from the authors of ref. [8].  The new
   version now reads:

"The question of what will be possible to learn from the DSN$\nu$F
data in the precision phase, and how well, has received only limited
attention.  A initial study by Yuksel, Ando and Beacom [8] considered
specific examples with focus on the low statistics of GADZOOKS. The
main result was that GADZOOKS has a chance to test the neutrino
spectrum if the flux is close to the current SuperKamiokande limit.
The status of the art on what data from the DSN$\nu$F will tell us is
well summarized in the work by Fogli et al. [16], where a detailed
study of the background is presented for detection with pure water and
with water with Gadolinium."

2. I added a paragraph in sec. II, in reply to the referee's comment
   1).  This new paragraph is the third of sec. II, and reads:

``I have estimated the error associated with approximating a composite
spectrum with the form (1), in the case of maximal
permutation of the neutrino fluxes, which is realized (for
antineutrinos, of interest here) for the normal mass hierarchy, or for
the inverted hierarchy with $\sin^2 \theta_{13}\lta 3 \cdot 10^{-6}$
[17,18].  I assumed a difference in the
$\barnue$ and $\barnumu,\barnutau$ average energies up to $30\%$ and
up to a factor of two difference in the luminosities of the electron
and non electron flavors.  The result is that the error is smaller
than 6\% above 10 MeV of energy, if Eq. (1) is used with
$L$ and $E_0$ being the luminosity and the average energy of the
composite spectrum, and $\alpha$ chosen to reproduce the width of the
composite spectrum.''

3. The text immediately before and after Eq. (3) has been edited in
   reply to referee's comment 1). Specifically, I added a paragraph,
   which reads:

``Throughout the paper, the expression (3) will be used for the
DSN$\nu$F.  This formula is valid in the continuum limit, and only if
individual variations between different stars are negligible. This
last statement has not been checked in detail; it is however supported
by the results of numerical simulations [33]'' .  

The footnote [33] was already present in the first version, and has not been changed.

4. I added a paragraph at the very end of sec. III, to account for referee's comment 2).
   Its text is: 

``In closing this section, I would like to emphasize that, while useful
for understanding, the analytical approximations discussed here lose
validity below 15-20 MeV of energy.  Thus, to model observables at
these low energies, it is necessary to calculate the neutrino flux
numerically using Eq. (3).  I do so in the reminder of this
work.''

5. I modified fig. 5, and its caption, in reply to the referee's comment 3).

6. In reply to the referee's comment 3), I edited what was the last
   paragraph (now next-to-last) of sec. IV, and added a final paragraph.
   The edited part now reads:

``The figure also illustrates a possible measurement
of $N$ and $r$, with central values and 1$\sigma$ statistical errors
on these two quantities [37].  If only $r$ is considered -- for robustness
against uncertainties on $R_{SN}(0)\times L$ -- then for water only a
major portion of the parameter space is allowed within $1\sigma$, and
the entire space is within $3\sigma$. Instead, for water+Gd the
$1\sigma$ allowed region is much more restricted, and the $3\sigma$
region excludes the edges of the parameter space; for example, the
measurement of $r=1.2$ would exclude the point $E_0=12$ MeV and
$\alpha=4.5$.  Including the information on the number of events
reduces the allowed region substantially: while for pure water the
whole $\alpha- E_0$ plane is allowed within $3\sigma$, for water+Gd
the potential for exclusion is better. For the specific case in the
figure, a measurement of $N=200$ would exclude $E_0=12$ MeV regardless
of the value of $\alpha$.

Notice that the region allowed by $N$ is contained inside the one
allowed by $r$, meaning that the number of events alone is sufficient
to constrain the original neutrino spectrum, if $L$, $R_{SN}(0)$ and
$\beta$ are known very precisely.  In presence of errors on these
quantities, which is probably more realistic, the ratio $r$ will be
more constraining instead.''.  

The footnote [37] was added for consistency. Its text is: 

``For the number of events I have used the sum of the numbers of
events in the first three (four) energy bins for pure water
(water+Gd). The higher energy bins are background-dominated and thus
including them would increase the error on the signal. ''

7. I added ref. [13], thus addressing the referee's comment 4).

---------------------------------------------------------------

Reply to the referee's comments:

> 1) It is clear that some assumptions are taken implicitly into account.
> For example, it has been supposed that all the supernovae have the same
> initial spectrum. The fact that different supernovae can can behave
> differently can be a further source of uncertainty. This fact should be
> stressed by the author. Moreover, the effect of oscillations are not
> considered in the calculation. As pointed out by the author, the
> Raffelt-Janka formula is still a good approximation for high energy
> neutrinos, but the paper lack of an estimation of the uncertainty
> induced by oscillation effect. This can be done considering the
> differences between the limiting cases of theta_13=0 and theta_13 large,
> both in normal and in inverted mass hierarchy.

I edited the text to give more emphasis to the uncertainty due to
individual differences between supernovae. The new text is the next
paragraph after Eq. (3) and is copied above in the summary of changes.

I have also estimated the size of the error associated with using the
Raffelt-Janka formula to approximate a composite antineutrino
spectrum, for the worst case scenario of maximal permutation of
spectra, realized, in the case of antineutrinos, for small theta_13
and inverted mass hierarchy, or normal hierarchy. I find an error
smaller than 6% above 10 MeV of energy.  Details are given in the new
paragraph that I have added, the third of sec. II (see summary of changes). 

> 2) It should be stressed that the analytical approximation in sec. III
> as well as the exponential fit in Eq. (9) are not a good approximation
> at lower energies but gives only the correct asymptotic behavior at
> large energies. They should not be used for calculations but only for
> the understanding of the high energy tail of the spectrum.

All my results were obtained with the exact formula, eq. (3), which I
evaluated numerically.  To stress this, and that the analytics is only
for understanding, I added the last paragraph of  sec. III (copied
above in the summary of changes).

> 3) In my opinion, it would be very interesting to show a figure similar
> to fig. 5 in which, in one or two cases of "simulated" values of E_0 and
> alpha, the allowed bands (say, at 1sigma) for r and N are shown, both
> for pure-water and for Gd-loaded detectors. The overlap of these two
> bands would be the "allowed solution" for the two parameters. This
> figure would clarify the effective sensitivity to the spectral
> parameters and show that this sensitivity would be dramatically improved
> in the case of Gd-loaded water.

I have done the study suggested in this comment, and found it
illuminating, indeed.  The results are given in the updated fig. 5
(the figure caption was updated as well) and in the text that refers
to this figure, which I edited for consistency.  The new text is also
copied above in the summary of changes.

> 4) Finally, ref. [12] should also be integrated by the recent paper by
> Wurm et al., Phys. Rev. D75 023007, 2007 (astro-ph/0701305).

I added this reference, which is now reference [13].

